An Algebra Containing the Two-Sided Convolution Operators

We present an intrinsically defined algebra of operators containing the right and left invariant Calder\'on-Zygmund operators on a stratified group. The operators in our algebra are pseudolocal and bounded on L^p (1<p<\infty). This algebra provides an example of an algebra of singular integrals that falls outside of the classical Calder\'on-Zygmund theory.

==> remarkonassump.tex <==
In Section \ref{SectionNewDist}, we studied two lists of vector
fields ($X_1, \ldots, X_p$ and $Y_1,\ldots, Y_q$) such that
$\l[ X_j, Y_k\r]=0$ for all $j,k$, and both the $X_j$s and
the $Y_k$s span the tangent space at every point.  There
is one obvious example of two such lists of vector fields:
let the $X_j$ span the right invariant vector fields on some
Lie group, and let the $Y_k$ span the left invariant
vector fields on the same Lie group.  In fact, in this paper,
we will be taking the Lie group to be $G$.  The point of this
section will be to show that this is the only such example.  This is a
bit of a deviation from the main line of reasoning of the rest
of the paper (and so can be skipped on a first reading).  However,
we justify its inclusion as follows:  Theorem \ref{ThmNewDist}
is the crux of this paper, and this section shows that we are
using it (nearly) to the fullest extent possible.  Ie, there may be
a way to extend some of
our results to other Lie groups, but to go any
further than that, one would need a replacement for Theorem \ref{ThmNewDist}.

Our setup is as follows: we consider $X_j, Y_k$ as above on some
connected open set $\Omega\subset \R^d$.  Let $\lieh$ be the
Lie subalgebra of vector fields on $\Omega$, generated by the $Y_k$.
\begin{lemma}\label{LemmaCommuteTranslate}
Fix $\xi\in \Omega$.  Any linear dependence at $\xi$ of $\lieh$ is
a linear dependence of $\lieh$ thought of as sections of $T\Omega$.  Ie, if $Z_1,\ldots, Z_m\in \lieh$,
and
$$\sum_{k=1}^m a_k Z_k\l( \xi\r)=0$$
then,
$$\sum_{k=1}^m a_k Z_k =0$$
where the $a_k$ are constants.
\end{lemma}
\begin{proof}
Suppose $\sum_{k=1}^m a_k Z_k\l( \xi\r)=0$.  Fix $\eta\in \Omega$.
We wish to show that $$\sum_{k=1}^m a_k Z_k\l( \eta\r)=0$$
Let
$$\Texp{\int_0^1 \sum_{j=1}^q b_j\l( s\r) X_j ds}\xi=\eta$$
which is always possible.  For $\xi'$ in a small neighborhood
of $\xi$, define:
$$\phi\l( \xi'\r)=\Texp{\int_0^1 \sum_{j=1}^q b_j\l(s\r) X_j ds}\xi'$$
Then $\phi$ defines a diffeomorhpism from a small neighborhood
of $\xi$ to a small neighborhood of $\eta$.  Since the $Y_k$s
commute with the $X_j$s (and hence, so do the $Z_k$s), it is easy to see:
$$d\phi\l( Z_k\r)\l( \eta\r) = Z_k\l( \eta\r)$$
and, thus, $\sum_{k=1}^m a_k Z_k\l( \eta\r) =0$.
\end{proof}
\begin{rmk}
In light of our goal, the proof of Lemma \ref{LemmaCommuteTranslate} is nothing
more than translating $\xi$ to $\eta$ by multiplication on the left.
\end{rmk}

Lemma \ref{LemmaCommuteTranslate} shows that $\lieh$ is $d$ dimensional.
Let $H$ be a Lie group whose Lie algebra is $\lieh$.  For $Z\in \lieh$,
we write $Z$ when we think of it as a section of $T\Omega$, and
$\Zt$ when we think of it as a left invariant vector field on $H$.

\begin{prop}\label{PropDiffeoToLieGroup}
For every $\xi\in \Omega$ there exists a neighborhood $U\subset \Omega$ of $\xi$,
a neighborhood $V\subset H$ of the identity, and a diffeomorphism $\phi:U\rightarrow V$,
such that $d\phi\l( Z\r) = \Zt$, for all $Z\in \lieh$.
\end{prop}

Proposition \ref{PropDiffeoToLieGroup} achieves our goal.  Indeed,
$d\phi\l( X_j\r)$ commutes with $\Zt$ for every $Z\in \lieh$,
and therefore, $d\phi\l(X_j\r)$ is a right invariant vector field on $V$,
for every $j$.

We sketch a proof of Proposition \ref{PropDiffeoToLieGroup} as
it is just a short exercise in differential topology, and
such results are surely well known.  Consider the manifold
$\Omega\times H$ and the integrable distribution on $\Omega\times H$ (in the
sense of Frobenius' theorem) given by $\l( Z, \Zt\r)$,
where $Z\in \lieh$.  By Frobenius' theorem, this gives rise
to a foliation of $\Omega\times H$.  In light of Lemma
\ref{LemmaCommuteTranslate} the leaves of this foliation
are (at least locally) graphs of diffeomorphisms with
the desired properties.

